On torsion-free modules and semi-hereditary rings

The class of semi-hereditary rings is an important class of rings in theories that do not assume the Noetherian condition, such as perfectoid ring theory. We prove several results concerning the structure theory of this class, focusing on the relationship between semi-hereditary rings and the flatness of torsion-free modules. We also consider Shimomoto's problem concerning the flatness of the Frobenius map.

==> m_syu_operator.tex <==
\def\m@syu@operatorloaded{loaded!}

\let\@xp\expandafter
\renewcommand{\hom}{\operatorname{Hom}} %defaultでは \hom -> hom

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\lt}{\operatorname{Lt}}
\newcommand{\Le}{\operatorname{Le}}
\newcommand{\lc}{\operatorname{Lc}}
\newcommand{\card}{\operatorname{Card}}
\newcommand{\z}{\operatorname{z}}
\newcommand{\Mn}{\operatorname{M}_n}
\newcommand{\gln}{\operatorname{GL}_n}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\orb}{\operatorname{Orb}}
\newcommand{\emb}{\operatorname{Emb}}
\newcommand{\aut}{\operatorname{Aut}}
\newcommand{\im}{\operatorname{Im}}
\newcommand{\map}{\operatorname{Map}}
\newcommand{\gal}{\operatorname{Gal}}
\newcommand{\hess}{\operatorname{Hess}}
\newcommand{\Int}{\operatorname{Int}}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\nil}{\operatorname{nil}}
\newcommand{\rad}{\operatorname{rad}}
\newcommand{\cl}{\operatorname{Cl}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\ann}{\operatorname{Ann}}
\newcommand{\bil}{\operatorname{Bil}}
\newcommand{\spec}{\operatorname{Spec}}
\newcommand{\spm}{\operatorname{Spm}}
\newcommand{\ass}{\operatorname{Ass}}
\newcommand{\supp}{\operatorname{Supp}}
\newcommand{\ob}{\operatorname{Ob}}
\newcommand{\pic}{\operatorname{Pic}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\clg}{\operatorname{Cl}}
\newcommand{\idht}{\operatorname{ht}}
\newcommand{\coht}{\operatorname{coht}}
\newcommand{\trdeg}{\operatorname{tr\text{.}deg}}
\newcommand{\emdim}{\operatorname{em\text{.}dim}}
\newcommand{\spa}{\operatorname{sp}}
\newcommand{\proj}{\operatorname{Proj}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\coker}{\operatorname{Coker}}
\newcommand{\coim}{\operatorname{Coim}}
\newcommand{\Ch}{\operatorname{Ch}}
\newcommand{\coch}{\operatorname{CoCh}}
\newcommand{\mult}{\operatorname{mult}}
\newcommand{\cacl}{\operatorname{CaCl}}
\newcommand{\Min}{\operatorname{Min}}
\newcommand{\Max}{\operatorname{Max}}
\newcommand{\Char}{\operatorname{Char}}
\newcommand{\prjdim}{\operatorname{prj\text{.}dim}}
\newcommand{\injdim}{\operatorname{inj\text{.}dim}}
\newcommand{\E}{E}%%松村，BHは斜体にしている
\newcommand{\mdepth}{\operatorname{depth}}
\newcommand{\gldim}{\operatorname{gl\text{.}dim}}
\newcommand{\gr}{\operatorname{gr}}
\newcommand{\grade}{\operatorname{grade}}
\newcommand{\pr}{\operatorname{pr}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Nat}{\operatorname{Nat}}
\newcommand{\Func}{\operatorname{Func}}
\newcommand{\htone}{\operatorname{Ht1}}
\newcommand{\der}{\operatorname{Der}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\grmod}{\operatorname{gr\text{-}Mod}}
\newcommand{\prj}{\operatorname{Prj}}
\newcommand{\inj}{\operatorname{Inj}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\pgrade}{\operatorname{p\text{-}grade}}
\newcommand{\fmod}{\operatorname{mod}}
\newcommand{\fp}{\operatorname{fp}}
\newcommand{\tot}{\operatorname{Tot}}
\newcommand{\G}{\operatorname{G}}
\newcommand{\bigrank}{\operatorname{big\ rank}}
\newcommand{\wdim}{\operatorname{w\text{.}dim}}
\newcommand{\fprjdim}{\operatorname{f\text{.}gl\text{.}dim}}
\newcommand{\wgldim}{\operatorname{w\text{.}gl\text{.}dim}}
\newcommand{\fdim}{\operatorname{f\text{.}dim}}
%%%%%
%%%%%一時的な措置？科研費LaTeXと衝突
\@ifundefined{soc}
	{\newcommand{\soc}{\operatorname{Soc}}}
	{\newcommand{\socle}{\operatorname{Soc}}
	\PackageWarning{askw.sty}{\protect\soc\space is defineb by KAKENHI LaTeX. so I define \protect\socle\space instead.}}
%%%%%

\newcommand{\middleoplus}{\mathchar"134C{}}

\let\midoplus\middleoplus

\newcommand{\newmax}{\mathop\textrm{max}\limits}
\newcommand{\newmin}{\mathop\textrm{min}\limits}
\newcommand{\newsup}{\mathop\textrm{sup}\limits}
\newcommand{\newinf}{\mathop\textrm{inf}\limits}

\newcommand{\ilim}[1][\relax]{%
	\def\ilim@chk{#1}%
	\@xp\ifx\ilim@chk\relax
		\varinjlim
	\else
		\mathop{\varinjlim}\limits_{#1}%
	\fi}
\newcommand{\plim}[1][\relax]{%
	\def\plim@chk{#1}%
	\@xp\ifx\plim@chk\relax
		\varprojlim
	\else
		\mathop{\varprojlim}\limits_{#1}%
	\fi}

\newcommand{\opcat}[1]{\mathscr{#1}^{\mathrm{op}}}

\@ifundefined{C}{\newcommand{\C}{\mathbb{C}\PackageWarning{askw.sty}{Use \protect\Co\space instead \protect\C\space.}} %%%LuaTeX ではhyperrefと衝突！
}{}

\newcommand{\A}{\mathbb{A}}
\newcommand{\Co}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\F}{\mathbb{F}}

\newcommand{\oka}[1][O]{%%%% mathrsfsが読み込まれていない可能性を考慮
	\ifx\mathscr\@undefined
		\PackageError{askw.sty}{\protect\oka\space needs to be loaded mathrsfs package.}\@ehd
	\else
		\mathscr{#1}%
	\fi
}

\newcommand{\ideal}[1]{\mathfrak{#1}}

\newlength\masyulengtha
\newlength\masyulengthb
\newlength\masyulengthc
